Inequality constraints in variational quantum circuits with qudits

Quantum optimization is emerging as a prominent candidate for exploiting the capabilities of near-term quantum devices. Many application-relevant optimization tasks require the inclusion of inequality constraints, usually handled by enlarging the Hilbert space through the addition of slack variables. This approach, however, requires significant additional resources especially when considering multiple constraints. Here, we study an alternative direct implementation of these constraints within the QAOA algorithm, achieved using qudit-SUM gates, and compare it to the slack variable method generalized to qudits. We benchmark these approaches on three paradigmatic optimization problems. We find that the direct implementation of the inequality penalties vastly outperforms the slack variables method, especially when studying real-world inspired problems with many constraints. Within the direct penalty implementation, a linear energy penalty for unfeasible states outperforms other investigated functional forms, such as the canonical quadratic penalty. The proposed approach may thus be an enabling step for approaching realistic industry-scale and fundamental science problems with large numbers of inequality constraints.

==> numerics/numerics_header.tex <==
\section{Numerical benchmarks} \label{sec: numerics}
In this section, we show numerical results for QAOA performed  in different scenarios where inequality constraints play a role. First, we analyse the ability of QAOA to sample feasible solutions for a generic random spin model [ ]. Then we show how to construct a starting constrained state for warm start QAOA and in the end we test the performance on the industry relevant problem of electric vehicle (EV) charging[ ], which is subject to multiple constraints. For all of these problems, we compare the performance of the constraint handling methods described in sections ~\ref{sec:slack},~\ref{sec: penalties}. Simulations are performed using the Powell classical optimizer. \seb{For each problem instance we perform $N_\mathrm{runs}=XX$ separate runs where for each run the } parameters are initialized randomly in the interval $[0,2\pi]$. \seb{For each finished QAOA run, we extract the classical solutions of the optimization  problem by sampling $N_S=XX$ solutions from the quantum state $\ket{...}$. }
\subsection{Metrics}
We consider the three metrics described in the following section.

The success rate is defined as 
\begin{equation}
    r = \frac{N_{\mathrm{sampled}}}{N_{\mathrm{runs}}}
\end{equation}
where $N_{\mathrm{sampled}}$ is the number of times the constrained ground state is sampled over a total number $N_{\mathrm{runs}}$ of runs. We define the approximation ratio as 
\begin{equation}
    R = \underset{\mathrm{samples}}{\mathrm{Min}}\frac{E_{\mathrm{samp}}-E_0}{|E_0|}
\end{equation}
where $E_{\mathrm{samp}}$ is the energy of the sampled state and $E_0$ is the constrained state with the lowest energy. This is due to the fact that QAOA is mostly studied in order to understand its efficiency in solving industrial optimization problems, for which we care about the energy of a single configuration and not the average over the final state. A third figure of merit, related to the ability of these penalties to sample constrained solutions, is the total weight of constrained solutions present in the final state:
\begin{align*}
    &\ket{\psi(\boldsymbol{\alpha^*,\beta^*})} = \sum_{x}c_x(\boldsymbol{\alpha^*,\beta^*})\ket{\boldsymbol{x}}\\
    & W= \sum_{\boldsymbol{x}\in \mathrm{feasible}}|c_x(\boldsymbol{\alpha^*,\beta^*})|^2.
\end{align*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure*}
    \centering
    \includegraphics[width = 0.47\textwidth]{images/rates_approx/boxplot_rate_approx_penalty_4.0.jpeg}
    \includegraphics[width = 0.47\textwidth]{images/boxplot_rate_approx_penalty_-4.0.jpeg}
    \caption{Success rates $r$ and approximation ratios $R$ for single layer QAOA and three types of penalty functions for a system of nine qubits. The box plots shows statistics for averages over 20 different instances of the random Hamiltonian of Eq.~\eqref{eq:skrandom}, with couplings $J_{ij}$ distributed as a Gaussian with mean $0$ and variance $1$ and 50 runs per single Hamiltonian. The results are shown as a function of the total spin imposed on the system (hence x-axis has coordinates from $-4.5$ and $4.5$. a) The results for the three types of penalties ~\eqref{eq:flat},~\eqref{eq:linear},~\eqref{eq:quadratic} become more similar as the value of $S_0$ increases. This is due to the fact that for high target values the system becomes more and more unconstrained, hence the different type of penalties will have less impact on the system. b) Same figures of merit but for runs using slack variables}
    \label{fig:success rate}
\end{figure*}


\input{numerics/random}
\input{numerics/sampling}
\input{numerics/Ev}
